The x86isa Books: Features, Usage, and Future Plans

The x86isa library, incorporated in the ACL2 community books project, provides a formal model of the x86 instruction-set architecture and supports reasoning about x86 machine-code programs. However, analyzing x86 programs can be daunting -- even for those familiar with program verification, in part due to the complexity of the x86 ISA. Furthermore, the x86isa library is a large framework, and using and/or contributing to it may not seem straightforward. We present some typical ways of working with the x86isa library, and describe some of its salient features that can make the analysis of x86 machine-code programs less arduous. We also discuss some capabilities that are currently missing from these books -- we hope that this will encourage the community to get involved in this project.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Warren Hunt Jr.\ and Anna Slobodova (Eds.):\\
ACL2 Theorem Prover and its Applications\\
EPTCS 249, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.249.1}{10.4204/EPTCS.249.1}}
\pdfoutput=1

